Stronger L2/L2 Compressed Sensing; Without Iterating

We consider the extensively studied problem of $\ell_2/\ell_2$ compressed sensing. The main contribution of our work is an improvement over [Gilbert, Li, Porat and Strauss, STOC 2010] with faster decoding time and significantly smaller column sparsity, answering two open questions of the aforementioned work. Previous work on sublinear-time compressed sensing employed an iterative procedure, recovering the heavy coordinates in phases. We completely depart from that framework, and give the first sublinear-time $\ell_2/\ell_2$ scheme which achieves the optimal number of measurements without iterating; this new approach is the key step to our progress. Towards that, we satisfy the $\ell_2/\ell_2$ guarantee by exploiting the heaviness of coordinates in a way that was not exploited in previous work. Via our techniques we obtain improved results for various sparse recovery tasks, and indicate possible further applications to problems in the field, to which the aforementioned iterative procedure creates significant obstructions.

==> fourier.tex <==
\section{Sparse Fourier transform}\label{sec:fourier}

\subsection{Formal Statement of the Theorem}
Our last result concerns the ubiquitous problem of frequency estimation from Fourier measurements. For any vector $x \in \C^n$, let $\wh{x} \in \C^n$ denote the discrete Fourier transform of $x$.
The only previous known result by the breakthrough work of \cite{k17} achieves sample complexity $O(k/\epsilon)$ and running time $O(\epsilon^{-1} k \log^{2.001} n \log R^*)$ for $\ell_2/\ell_2$ Fourier set query. Here, $R^*$ is an upper bound on the $\|\cdot\|_{\infty}$ norm of the vector, in most applications being considered $\poly(n)$. We indicate how the approach  for set-query described in the previous section immediately gives an algorithm with $O(k\log n/ \epsilon)$ running time. The result we get has no dependence on the running time on $\log R^*$, but does not achieve the optimal sample complexity.
\vspace{-2mm}
\begin{theorem}[Fourier set query]\label{thm:main_fourier_I}
Given a vector $x \in \C^n$, for every $\epsilon \in (0,1)$ and $k \geq 1$, any $S \subseteq [n]$, $|S| = k$, there exists an algorithm that takes $O(\epsilon^{-1} k \log (n/\delta))$ samples, runs in $O(\epsilon^{-1} k \log (n/\delta))$ time, and outputs a vector $x' \in \C^n$ such that
$
\| (x' - \wh{x})_S \|_2^2 \leq \epsilon \| \wh{x}_{[n] \backslash S } \|_2^2 + \delta \| \wh{x} \|_1^2
$
holds with probability at least $9/10$.
\end{theorem}


We present some definitions and backgrounds of Fourier transform in Section~\ref{sec:fourier_definitions_and_backgrounds}.
Then we introduce spectrum permutations and filter functions in Section~\ref{sec:fourier_permutation_and_filter_function}. They are used as hashing schemes in Fourier transform literatures.
In Section~\ref{sec:fourier_collison_offset_noise}, we introduce collision events. large offset events, and large noise events.
We give a new algorithm and provide iterative loop analysis in Section~\ref{sec:fourier_iterative_loop_analysis}.
Finally, we present main result in Section~\ref{sec:fourier_main_result}.


\subsection{Definitions and some backgrounds of Fourier transform}\label{sec:fourier_definitions_and_backgrounds}

We use $\i$ to denote $\sqrt{-1}$. Note that $e^{\i \theta} = \cos(\theta) + \i \sin(\theta)$. For any complex number $z\in \C$, we have $z = a + \i b$, where $a,b \in \R$. We define the complement of $z$ as $\ov{z} = a - \i b$. We define $|z| = \sqrt{ z\ov{z} } = \sqrt{a^2 +b^2}$. For any complex vector $x\in \C^n$, we use $\supp(x)$ to denote the support of $x$, and then $\| x \|_0 = |\supp(x)|$. 

The discrete convolution of functions $f$ and $g$ is given by,
\begin{align*}
(f * g) [n] = \sum_{m = -\infty}^{+\infty} f[m] g[n-m]
\end{align*}

For a complex vector $x \in \C^n$, we use $\wh{x} \in \C^n$ to denote its Fourier spectrum,
\begin{align*}
\wh{x}_i = \frac{1}{\sqrt{n}} \sum_{j=1}^n e^{-2\pi \i i j/ n} x_j, \forall i\in [n].
\end{align*}

Then the inverse transform is
\begin{align*}
x_j = \frac{1}{\sqrt{n}} \sum_{i=1}^n e^{2\pi \i i j/ n} \wh{x}_i, \forall j \in [n].
\end{align*}

We define
\begin{align*}
\Err(x,k) = \min_{k-\sparse~y} \| x - y \|_2.
\end{align*}

\subsection{Permutation and filter function}\label{sec:fourier_permutation_and_filter_function}
We use the same (pseudorandom) spectrum permutation as \cite{hikp12a},
\begin{definition}
Suppose $\sigma^{-1}$ exists mod $n$. We define the permutation $P_{\sigma,a,b}$ by
\begin{align*}
(P_{\sigma,a,b} x)_i = x_{\sigma(i-a)} e^{-2\pi \i \sigma b i /n }.
\end{align*}
\end{definition}
We also define $\pi_{\sigma,b} = \sigma(i-b) \pmod n$. Then we have
\begin{claim}
$\wh{P_{\sigma,a,b} x}_{\pi_{\sigma,b}(i)} = \wh{x}_i e^{-2\pi \i \sigma a i /n}$.
\end{claim}
 $h_{\sigma,b}(i) = \text{round}(\pi_{\sigma,b}(i) B / n)$ and $o_{\sigma,b}(i) = \pi_{\sigma,b}(i) - h_{\sigma,b}(i) n /B$. We say $h_{\sigma,b}(i)$ is the ``bin'' that frequency $i$ is mapped into, and $o_{\sigma,b}(i)$ is the ``offset''.



We use the same filter function as \cite{hikp12a,ps15,ckps16},
\begin{definition}
Given parameters $B\geq 1$, $\delta >0$, $\alpha >0$. We say that $(G,\wh{G}') = (G_{B,\delta,\alpha}, \wh{G}'_{B,\delta,\alpha}) \in \R^n$ is a filter function(Figure~\ref{fig:filter_G}) if it satisfies the following properties \\
\begin{align*}
\rm{(\RN{1})} & ~ |\supp(G)| = O( \alpha^{-1} B \log (n/\delta)) , \\
\rm{(\RN{1})} & ~ \wh{G}'_i = 1, &\text{~if~} |i| \leq (1-\alpha) n / (2B), \\
\rm{(\RN{2})} & ~ \wh{G}'_i = 0, &\text{~if~} |i| \geq n / (2B), \\
\rm{(\RN{3})} & ~ \wh{G}'_i \in [0,1], &\text{~for~all~} i, \\
\rm{(\RN{4})} & ~ \left\| \wh{G}' - \wh{G} \right\|_{\infty} < \infty.
\end{align*}
\end{definition}

\begin{figure}[t]
\centering
	\includegraphics[width = 0.7\textwidth]{G}
	\caption{Filter $\wh{G}'$}\label{fig:filter_G}
\end{figure}


\subsection{Collision event, large offset event, and large noise event}\label{sec:fourier_collison_offset_noise}

We use three types of events defined in \cite{hikp12a} as basic building blocks for analyzing Fourier set query algorithms. 
For any $i\in S$, we define three types of events associated with $i$ and $S$ and defined over the probability space induced by $\sigma$ and $b$:
\begin{definition}[Collision, large offset, large noise]
``Collision'' event $E_{\mathrm{coll}}(i)$ : holds iff $h_{\sigma,b}(i) \in h_{\sigma,b}(S \backslash \{i\} )$.\\ ``Large offset'' event $E_{\mathrm{off}}(i)$ : holds iff $|o_{\sigma,b}(i)| \geq (1-\alpha) n / (2B)$. \\ ``Large noise'' event $E_{\mathrm{noise}}(i)$ : holds iff 
\begin{align*}
\E\left[ \left\| \wh{x}'_{ h^{-1}_{\sigma,b} ( h_{\sigma,b}(i) ) \backslash S } \right\|_2^2 \right] \geq \Err^2( \wh{x}', k ) / (\alpha B).
\end{align*}
\end{definition}

\begin{claim}[Claim 3.1 in \cite{hikp12a}]\label{cla:claim_3.1_hikp12a}
For any $i\in S$, the event $E_{\mathrm{coll}}(i)$ holds with probability at most $4 |S| / B$.
\end{claim}

\begin{claim}[Claim 3.2 in \cite{hikp12a}]\label{cla:claim_3.2_hikp12a}
For any $i\in S$, the event $E_{\mathrm{off}}(i)$ holds with probability at most $\alpha$.
\end{claim}

\begin{claim}[Claim 4.1 in \cite{hikp12a}]\label{cla:claim_4.1_hikp12a}
For any $i\in S$, $\Pr[ E_{\mathrm{noise} (i) } ] \leq 4 \alpha$.
\end{claim}

\begin{lemma}[Lemma 4.2 in \cite{hikp12a}]\label{lem:lemma_4.2_hikp12a}
Let $a \in [n]$ uniformly at random, $B$ divide $n$, and the other parameters be arbitrary in 
\begin{align*}
\wh{u} = \textsc{HashToBins}(x,\wh{z}, P_{\sigma,a,b}, B, \delta, \alpha).
\end{align*}
Then for any $i\in [n]$ with $j = h_{\sigma,b}(i)$ and none of $E_{\mathrm{coll}}(i)$, $E_{\mathrm{off}}(i)$ or $E_{\mathrm{noise}}(i)$ holding,
\begin{align*}
\E \left[ \left| \wh{u}_j - \wh{x}'_i e^{- \frac{2 \pi \i}{n} a \sigma i} \right|^2 \right] \leq 2 \frac{\rho^2}{\alpha B}.
\end{align*}
\end{lemma}

\begin{lemma}
Suppose $B$ divides $n$. The output $\wh{u}$ of $\textsc{HashToBins}$ satisfies
\begin{align*}
\wh{u}_j = \sum_{h_{\sigma,b}(i) = j} \wh{(x-z)}_i (\wh{G'_{B,\delta,\alpha}})_{-o_{\sigma,b}(i)} \omega^{a \sigma i} \pm \delta \| \wh{x} \|_1.
\end{align*}
Let $\zeta = | \{ i \in \mathrm{supp}(\wh{z}) ~|~ E_{\mathrm{off}}(i) \} |$. The running time of \textsc{HashToBins} is $O(\frac{B}{\alpha} \log (n/\delta) + \| \wh{z} \|_0 + \zeta \log (n/\delta) )$.
\end{lemma}


%\subsection{Fourier set query from previous work}
\begin{comment}
This section states the previous result in \cite{hikp12a} and provides a full proof for the completeness. Note that the following theorem is not explicitly stated in \cite{hikp12a}, but it is clearly follows from the proof in Lemma 4.8 and Theorem 4.9 in \cite{hikp12a}.
\begin{theorem}[Lemma 4.8 and Theorem 4.9 in \cite{hikp12a}]
Given a vector $x \in \C^n$, for every $\epsilon \in (0,1)$ and $k\geq 1$, any $S \subseteq [n]$, $|S| = k$, there exists an algorithm that takes 
\begin{align*}
O(\epsilon^{-1} k \log (n/\delta) \log (1/\epsilon) )
\end{align*}
samples, runs in 
\begin{align*}
O(\epsilon^{-1} k \log (n/\delta) \log (1/\epsilon) )
\end{align*}
time, and outputs a vector $x'\in \C^n$ such that
\begin{align*}
\| ( x' - \wh{x} )_S  \|_2^2 \leq \epsilon \| \wh{x}_{ [n] \backslash S} \|_2^2,
\end{align*}
holds with probability at least $9/10$.
\end{theorem}

\begin{proof}
Note that $\epsilon_r = f_r \epsilon$, $\alpha_r = \Theta(f_r^2)$, $f_r = O(1/r^2)$, $B_r = O(\epsilon^{-1} k \alpha_r f_r)$ and $R = \log k / \log k \log k$.

{\bf Proof of Sample Complexity.}

The sample complexity of \textsc{Estimation} is
\begin{align*}
& ~ \sum_{r=1}^R (B_r / \alpha_r) \log (n/\delta) \cdot \log (1/ (\alpha_r \epsilon_r) ) \\
\lesssim & ~ \sum_{r=1}^R (\epsilon^{-1} k f_r) \log (n/\delta) \cdot \log (1/ (\alpha_r \epsilon_r) ) \\
\lesssim & ~ \sum_{r=1}^R (\epsilon^{-1} k f_r) \log (n/\delta) \cdot \log (1 / (f_r^3 \epsilon)) \\
= & ~ \epsilon^{-1} k \log (n/\delta) \sum_{r=1}^R f_r ( \log(1/\epsilon) + 3 \log(f_r) ) \\
\lesssim & ~ \epsilon^{-1} k \log (n/\delta)
\end{align*}
where the first step follows by definition of $B_r$ and $\alpha_r$, the second step follows by definition of $\alpha_r$ and $\epsilon_r$, and the last step follows by $\sum_{r=1}^R f_r \leq O(1)$ and $\sum_{r=1}^R 3 f_r \log (f_r) \leq O(1)$.
\end{proof}
\end{comment}


\subsection{Iterative loop analysis}\label{sec:fourier_iterative_loop_analysis}

Iterative loop analysis for Fourier set query is more tricky than the classic set query, because in the Fourier case, hashing is not perfect, in the sense that by using spectrum permutation and filter function (as the counterpart of hashing techniques), one coordinate can non-trivially contribute to multiple bins. We give iterative loop induction in Lemma~\ref{lem:iterative_loop_analysis_fourier_set_query_I}.

\begin{lemma}\label{lem:iterative_loop_analysis_fourier_set_query_I}
Given parameters $C \geq 1000$, $\gamma \leq 1/1000$. For any $k\geq 1 , \epsilon \in (0,1)$, $R\geq 1$.
For each $i \in [R]$, we define
\begin{align*}
k_i = k \gamma^i, \epsilon_i =  \epsilon (10\gamma)^i, \alpha_i = 1/(200 i^3) , B_i = C \cdot k_i/ (\alpha_i^2 \epsilon_i ).
\end{align*}
For each $i\in [R]$:\\
If for all $j \leq [i-1]$ we have
\begin{align*}
\supp( \wh{w}^{(j)} ) \subseteq S_j, \quad | S_{j+1} | \leq k_{j+1}, \quad \wh{z}^{(j+1)} = \wh{z}^{(j)} + \wh{w}^{(j)}, \quad \wh{x}^{(j+1)} = \wh{x} - \wh{z}^{(j+1)},
\end{align*}
and
\begin{align*}
\| \wh{x}_{\ov{S}_{j+1}}^{(j+1)} \|_2^2 \leq (1+\epsilon_j) \| \wh{x}_{\ov{S}_{j}}^{(j)} \|_2^2 + \epsilon_j \delta^2 n \| \wh{x} \|_1^2.
\end{align*}
Then, with probability $1- 10 \alpha_i / \gamma$, we have
\begin{align*}
\supp( \wh{w}^{(i)} ) \subseteq S_i, \quad | S_{i+1} | \leq k_{i+1}, \quad \wh{z}^{(i+1)} = \wh{z}^{(i)} + \wh{w}^{(i)}, \quad \wh{x}^{(i+1)} = \wh{x} - \wh{z}^{(i+1)},
\end{align*}
and
\begin{align*}
\| \wh{x}_{\ov{S}_{i+1}}^{(i+1)} \|_2^2  \leq (1+\epsilon_i) \| \wh{x}_{\ov{S}_{i}}^{(i)} \|_2^2  + \epsilon_i \delta^2 n \| \wh{x} \|_1^2.
\end{align*}
\end{lemma}




\begin{proof}

We consider a particular step $i$. We can condition on $ | S_i | \leq k_i$.


{\bf Collision.}
Using Claim~\ref{cla:claim_3.1_hikp12a}, for any $t \in S_{i}$, the event $E_{\mathrm{coll}}(t)$ holds with probability at most 
\begin{align*}
4 |S_{i} | / B_i \leq \frac{4 k_i}{ C k_i / (\alpha_i^2 \epsilon_i)  } = 4 \alpha_i^2 \epsilon_i /C \leq \alpha_i.
\end{align*}
It means
\begin{align*}
\Pr_{\sigma,b} \left[ E_{\mathrm{coll}}(t) \right] \leq \alpha_i.
\end{align*}

{\bf Large offset.}
Using Claim~\ref{cla:claim_3.2_hikp12a}, for any $t \in S_i$, the event $E_{\mathrm{off}}(t)$ holds with probability at most $\alpha_i$, i.e.
\begin{align*}
\Pr_{\sigma,b} \left[ E_{\mathrm{off}}(t) \right] \leq \alpha_i.
\end{align*}

{\bf Large noise.}
Using Claim~\ref{cla:claim_4.1_hikp12a}, for any $t \in S_i$,
\begin{align*}
\Pr_{\sigma,b}[ E_{\mathrm{noise}}(t) ] \leq 4 \alpha_i.
\end{align*}

We say a coordinate $t$ is ``well isolated'' if none of the above three events holding.
By a union bound over the above three events, we have $t$ is ``well isolated'' with probability at least $1-6\alpha_i$.

Therefore, each $t\in S_i$ lies in $T_i$ with probability at least $1- 6 \alpha_i$. Then by Markov's inequality, we have $|S_i \backslash T_i| \leq \gamma k_i$ with probability $1- 6 \alpha_i/\gamma$. By definition $S_{i+1} = S_i \backslash T_i$, then we know that
\begin{align*}
| S_{i+1} | = | S_i \backslash T_i| \leq \gamma k_i \leq k_{i+1}.
\end{align*}

\begin{comment}
We define $\rho^{(i)}$ and $\mu^{(i)}$ as follows
\begin{align*}
\rho^{(i)} = & ~ \left\| \wh{x}^{(i)}_{\ov{S}_i} \right\|_2^2 + \delta^2 n \| \wh{x} \|_1^2 , \\
\mu^{(i)}  = & ~ \frac{\epsilon_i}{k_i} \left( \left\| \wh{x}^{(i)}_{\ov{S}_i} \right\|_2^2 + \delta^2 n \| \wh{x} \|_1^2 \right).
\end{align*}
\end{comment}
{\bf Upper bound $\| \wh{x}_{\ov{S}_i}^{(i)} \|_2^2$.} By Lemma statement we have
\begin{align}\label{eq:fourier_set_query_I_upper_bound_ovSi}
\| \wh{x}^{(i)}_{\ov{S}_i } \|_2^2 \leq & ~ (1+\epsilon_i) \| \wh{x}_{\ov{S}_i}^{(i)} \|_2^2 + \epsilon_i \delta^2 n \| \wh{x} \|_1^2 \notag \\
\leq & ~ (1+\epsilon_i) (1+\epsilon_{i-1}) \| \wh{x}_{\ov{S}_{i-1}}^{(i-1)} \|_2^2 + ( (1+\epsilon_i) \epsilon_{i-1} + \epsilon_i ) \delta^2 n \| \wh{x} \|_1^2 \notag \\
\leq & ~ \cdots \notag \\
\leq & ~ \prod_{j=1}^i (1+\epsilon_j) \| \wh{x}_{\ov{S}} \|_2^2 + \sum_{j=1}^i \epsilon_j \delta^2 n \| \wh{x} \|_1^2 \prod_{l = j+1}^i (1+\epsilon_l) \notag \\
\leq & ~ 8 ( \| \wh{x}_{\ov{S}} \|_2^2 +  \delta^2 n \| \wh{x} \|_1^2 ),
\end{align}

where the third step refers to recursively apply the second step, the last step follows by a geometric sum.

\begin{comment}
Using Lemma~\ref{lem:lemma_4.2_hikp12a}, we can calculate the expectation of $\| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \|_2^2$,
\begin{align*}
\E_a \left[ \left\| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \right\|_2^2 \right]
\leq & ~ |T_i| 2  \frac{\rho^{(i)}}{\alpha_i B_i}  \\
\leq & ~ |T_i| 2 \mu^{(i)} \frac{k_i}{\epsilon_i \alpha_i B_i} & \text{~by~} \rho^{(i)} = \frac{k_i}{\epsilon_i} \mu^{(i)} \\
\leq & ~ |T_i| 2 \mu^{(i)} \alpha_i  /C & \text{~by~} B_i = C k_i/ (\epsilon_i \alpha_i^2)\\
\leq & ~ |T_i| \mu^{(i)} \alpha_i /20 & \text{~by~} C \geq 40 \\
\leq & ~ k_i \mu^{(i)} \alpha_i. & \text{~by~} |T_i| \leq k_i 
\end{align*}
\end{comment}
For a fixed $t\in S_i$, let $j = h_{\sigma,b}(t)$.
By Lemma 3.3, we have
\begin{align*}
\wh{u}_j - \wh{x}_{t}^{(i)} \omega^{a\sigma t} = \sum_{t'\in T_i} \wh{G}'_{-o_{\sigma}(i')} \wh{x}_{t'}^{(i)} \omega^{a\sigma t'} \pm \delta \| \wh{x} \|_1
\end{align*}

For each $t \in S_i$, we define set $Q_{i,t} = h^{-1}_{\sigma,b}(j) \backslash \{t\}$.
Let $T_i$ be the set of coordinates $t \in S_i$ such that $Q_{i,t} \cap S_i = \emptyset$. Then it is easy to observe that
\begin{align*}
\sum_{t \in T_i} \left| \sum_{t' \in Q_{i,t} } \wh{G}'_{-o_{\sigma}(t)} \wh{x}_{t'}^{(i)} \omega^{a\sigma t'} \right|^2 = & ~ \sum_{t \in T} \left| \sum_{t' \in Q_{i,t} \backslash S} \wh{G}'_{-o_{\sigma}(t')} \wh{x}_{t'}^{(i)} \omega^{a\sigma t'} \right|^2 \\
\leq & ~ \sum_{t \in S} \left| \sum_{t' \in Q_{i,t} \backslash S} \wh{G}'_{-o_{\sigma}(t')} \wh{x}_{t'}^{(i)} \omega^{a \sigma t'} \right|^2
\end{align*}

We can calculate the expectation of $\| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \|_2^2$,
\begin{align*}
\E_{\sigma,a,b} \left[ \left\| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \right\|_2^2 \right] 
= & ~ \E_{\sigma,a,b}\left[ \sum_{t\in T_i} \left\| \wh{x}_{t}^{(i)} - \wh{w}_t^{(i)} \right\|_2^2 \right] \\
\leq &  ~ \sum_{i \in S} 2 \E_{\sigma,a,b} \left[ \left| \sum_{i' \in Q_i \backslash S} \wh{G}'_{-o_{\sigma}(i)} \omega^{a\sigma i} \right|^2  \right] + \delta^2 \| \wh{x} \|_1^2  \\
\leq & ~ \sum_{t\in S_i} (\frac{1}{B_i} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 \| \wh{x} \|_1^2)\\
\leq & ~ \frac{|S_i|}{B_i} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 |S_i| \cdot \| \wh{x} \|_1^2 \\
\leq & ~ \frac{\epsilon_i \alpha_i^2}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 |S_i| \cdot \| \wh{x} \|_1^2,
\end{align*}

where the last step follows from $|S_i| \leq k_i$ and $B_i = C \cdot k_i / (\alpha_i^2 \epsilon_i)$. 

Then, using Markov's inequality, we have,
\begin{align*}
 \Pr \left[ \left\| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \right\|_2^2 \geq \frac{\epsilon_i \alpha_i}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 \frac{|S_i|}{\alpha_i} \| \wh{x} \|_1^2 \right] \leq \alpha_i.
\end{align*}

Note that
\begin{align*}
\frac{\epsilon_i \alpha_i}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 \frac{|S_i|}{\alpha_i} \| \wh{x} \|_1^2 \leq & ~ \frac{\epsilon_i}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 \frac{|S_i|}{\alpha_i} \| \wh{x} \|_1^2 \\
\leq & ~ \frac{\epsilon_i}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \frac{\epsilon_i}{C} \delta^2 B_i \| \wh{x} \|_1^2 \\
\leq & ~ \frac{\epsilon_i}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \frac{\epsilon_i}{C} \delta^2 n \| \wh{x} \|_1^2 \\
\leq & \frac{\epsilon_i}{20} ( \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 n \| \wh{x} \|_1^2 ),
\end{align*}

where the first step follows by $\alpha_i \leq 1$, the second step follows by $|S_i| \leq k_i = \epsilon_i B_i \alpha_i^2 / C$, the third step follows by $B_i \leq n$, the last step follows by $C \geq 1000$.

Thus, we have
\begin{align}\label{eq:fourier_set_query_I_noise}
 \Pr \left[ \left\| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \right\|_2^2 \leq  \frac{\epsilon_i}{20} ( \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 n \| \wh{x} \|_1^2 ) \right] \geq 1- \alpha_i.
\end{align}

Recall that $\wh{w}^{(i)} = \wh{z}^{(i+1)} - \wh{z}^{(i)} = \wh{x}^{(i)} - \wh{x}^{(i+1)} $. It is obvious that $\supp(\wh{w}^{(i)} ) \subseteq T_i$.

Conditioning on all coordinates in $T_i$ are well isolated and Eq.~\eqref{eq:fourier_set_query_I_noise} holds, we have
\begin{align*}
\| \wh{x}_{\ov{S}_{i+1}}^{(i+1)} \|_2^2 = & ~ \| ( \wh{x}^{(i)} - \wh{w}^{(i)} )_{\ov{S}_{i+1}} \|_2^2 \\
= & ~ \| \wh{x}^{(i)}_{\ov{S}_{i+1}} - \wh{w}^{(i)}_{\ov{S}_{i+1}} \|_2^2 \\
= & ~ \| \wh{x}^{(i)}_{\ov{S}_{i+1}} - \wh{w}^{(i)} \|_2^2 \\
= & ~ \| \wh{x}^{(i)}_{\ov{S}_{i} \cup T_i} - \wh{w}^{(i)} \|_2^2 & \text{~by~} S_i = T_i \cup S_{i+1} \\
= & ~ \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \|_2^2 & \text{~by~}\ov{S}_i \cap T_i = \emptyset \\
\leq & ~ \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \epsilon_i ( \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 n \| \wh{x} \|_1^2 ) & \text{~by~Eq.~\eqref{eq:fourier_set_query_I_noise}} \\
= & ~ (1+\epsilon_i)\| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \epsilon_i \delta^2 n \| \wh{x} \|_1^2. & \text{~by~definition~}\mu_{(i)}
\end{align*}

\end{proof}



\begin{comment}
\section{Fourier transform II}

\begin{theorem}[Theorem 1.1 in \cite{k17}]
For every $\epsilon \in (1/n,1), \delta \in (0,1/2), x \in \C^n$ and every integer $k\geq 1$, any $S \subseteq [n]$, $|S| = k$, if $\| x \|_{\infty} \leq R^* \cdot \| x_{[n] \backslash S} \|_2 / \sqrt{k}$, $R^* = n^{O(1)}$, an invocation of \textsc{Estimate}($\wh{x},S,k,\epsilon,R^*$) returns $x' \in \C^n$ such that
\begin{align*}
\| (x - x')_S \|_2^2 \leq \epsilon \| x_{[n] \backslash S} \|_2^2
\end{align*}
using $O_{\delta}( \epsilon^{-1} k )$ samples and $O_{\delta}( \epsilon^{-1} k \log^{3+\delta} n )$ time with at least $4/5$ success probability.
\end{theorem}
\end{comment}


\subsection{Main result}\label{sec:fourier_main_result}

\begin{algorithm}[t]
\begin{algorithmic}\caption{Fourier set query algorithm}\label{alg:fourier_set_query_I}
\Procedure{\textsc{FourierSetQuery}}{$x,S,\epsilon,k$}\Comment{Theorem~\ref{thm:fourier_set_query_I}}
	\State $\gamma \leftarrow 1/1000, C \leftarrow 1000$,
	$\wh{z}^{(1)} \leftarrow 0$, $S_1 \leftarrow S$
	\For{ $i=1 \to R$}
		\State $k_i \leftarrow k \gamma^i$, $\epsilon_i \leftarrow \epsilon (10\gamma)^i$, $\alpha_i \leftarrow 1/(100 i^3)$, $B_i \leftarrow C \cdot k_i / (\alpha_i^2 \epsilon_i)$
		\State $\wh{w}^{(i)}, T_i \leftarrow \textsc{EstiamteValues}(x,\wh{z}^{(i)},S_i,B_i,\delta,\alpha_i)$\Comment{$\wh{w}^{(i)}$ is $|T_i|$-sparse}
		\State $S_{i+1} \leftarrow S_i \backslash T_i$
		\State $\wh{z}^{(i+1)} \leftarrow z^{(i)} + \wh{w}^{(i)}$
	\EndFor
	\State \Return $\wh{z}^{(R+1)}$
\EndProcedure
\Procedure{\textsc{EstimateValues}}{$x,\wh{z},S,B,\delta,\alpha$} \Comment{Lemma~\ref{lem:iterative_loop_analysis_fourier_set_query_I}}
		\State Choose $a,b \in [n]$ uniformly at random
		\State Choose $\sigma$ uniformly at random from the set of odd numbers in $[n]$ 
		\State $\wh{u} \leftarrow \textsc{HashToBins}(x,\wh{z},P_{\sigma,a,b},B,\delta,\alpha)$
	\State $\wh{w} \leftarrow 0 $, $T\leftarrow \emptyset$
	\For{$t \in S$}
		\If{$t$ is isolated from other coordinates of $S$} \Comment{$h_{\sigma,b}(t) \notin h_{\sigma,b}(S \backslash \{t\})$}
			\If{no large offset} \Comment{$|o_{\sigma,b}(t)| < (1-\alpha) n /(2B)$}
				\State $\wh{w}_t \leftarrow \wh{u}_{h_{\sigma,b}(t)} e^{\frac{2\pi \i}{n} \sigma a t }$
				\State $T \leftarrow T \cup \{t\}$
			\EndIf
		\EndIf
	\EndFor
	\State \Return $\wh{w}, T$
\EndProcedure
\Procedure{\textsc{HashToBins}}{$x,\wh{z},P_{\sigma,a,b},B,\delta,\alpha$}
	\State Compute $\wh{y}_{jn/B}$ for $j\in [B]$, where $y = G_{B,\alpha,\delta} \cdot (P_{\sigma,a,b} x)$ 
	\State Compute $\wh{y}'_{jn/B} = \wh{y}_{jn/B} - ( \wh{G'_{B,\alpha,\delta} } * \wh{P_{\sigma,a,b} z} )_{jn/B}$ 
	\State \Return $\wh{u}_j = \wh{y}'_{jn/B}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

In this subsection, we give the main result as the following theorem.

\begin{theorem}[Main result]\label{thm:fourier_set_query_I}
Given a vector $x \in \C^n$, for every $\epsilon \in (0,1)$ and $k\geq 1$, any $S \subseteq [n]$, $|S| = k$, there exists an algorithm (Algorithm~\ref{alg:fourier_set_query_I}) that takes 
\begin{align*}
O(\epsilon^{-1} k \log (n/\delta)  )
\end{align*}
samples, runs in 
\begin{align*}
O(\epsilon^{-1} k \log (n/\delta) )
\end{align*}
time, and outputs a vector $x'\in \C^n$ such that
\begin{align*}
\| ( x' - \wh{x} )_S  \|_2^2 \leq \epsilon \| \wh{x}_{ [n] \backslash S} \|_2^2 + \delta \| \wh{x} \|_1^2,
\end{align*}
holds with probability at least $9/10$.
\end{theorem}
\begin{proof}
\begin{comment}
We show how to modify the parameter setting in \cite{hikp12a}. \cite{hikp12a} uses the the same shrinking factor $f_r$ for $\epsilon_r$ and $k_r$. Our idea is to use the different shrinking factor. We use shrinking factor $g_r$ for $k_r$ and $f_r$ for $\epsilon_r$. We choose $g_r / f_r = 1 / r^4$ and $f_r = \Theta(1/r^2)$ and $g_r = \Theta(1/r^6)$.

We choose $\epsilon_r = f_r \epsilon$, $\alpha_r = \Theta(f_r^2)$, $k_r = k \prod_{r=1}^R f_r$, $B_r = O(\epsilon^{-1} k \alpha_r f_r)$
\end{comment}
{\bf Proof of Sample Complexity.}
The sample complexity of \textsc{Estimation} is
\begin{align*} 
\sum_{i=1}^R (B_i / \alpha_i) \log (n/\delta) = \epsilon^{-1} k \log (n/\delta).
\end{align*}

{\bf Proof of Success Probability.}

The failure probability is
\begin{align*}
\sum_{i=1}^{R} 10 \alpha_i /\gamma < 1/10.
\end{align*}

{\bf Proof of Final Error}

\begin{align*}
 \| \wh{x}_S - \wh{z}^{(R+1)} \|_2^2 
= & ~ \sum_{i=1}^R \| \wh{x}_{T_i}^{(i)} - \wh{w}^{(i)} \|_2^2 \\
\leq & ~ \sum_{i=1}^R  k_i \mu^{(i)} /20 & \text{~by~Eq.~\eqref{eq:fourier_set_query_I_noise}} \\
\leq & ~ \sum_{i=1}^R \epsilon_i ( \| \wh{x}_{\ov{S}_i}^{(i)} \|_2^2 + \delta^2 n \| \wh{x} \|_1^2 )  /20 & ~\text{~by~Definition~of~} \mu^{(i)} \\
\leq & ~ \sum_{i=1}^R \epsilon_i \cdot 10( \| \wh{x}_{\ov{S}} \|_2^2 + \delta^2 n \| \wh{x} \|_1^2 )  /20 & \text{~by~Eq.~\eqref{eq:fourier_set_query_I_upper_bound_ovSi}} \\
\leq & ~ \epsilon (\| \wh{x}_{\ov{S}} \|_2^2 + \delta^2 n \| \wh{x} \|_1^2). & \text{by~geometric~sum}
\end{align*}

\end{proof}

\begin{comment}
\begin{table}[t]
\begin{center}
    \begin{tabular}{| l | l | l | l | l | l| l | l |}
    \hline
    Algorithm & $g_r$ & $f_r$ & $\epsilon_r$ & $\alpha_r$ & $k_r$ & $B_r$ \\ \hline
    \cite{hikp12a} & $\emptyset$ & $\Theta(1/r^2)$ & $f_r \epsilon$ & $\Theta(f_r^2)$ & $\prod_{i=1}^r f_r k$ & $C k \alpha_r f_r / \epsilon$ \\ \hline
    Our \cite{hikp12a} & $\Theta(1/r^6)$ & $\Theta(1/r^2)$ & $f_r \epsilon$ & $\Theta(f_r^2)$ & $\prod_{i=1}^r g_r k$ & $r^6 \cdot C k \alpha_r f_r/\epsilon$\\ \hline
    Our idea & $ \gamma^r $ & $ (10\gamma)^r $ & $ \gamma^r \epsilon$ & $\emptyset$ & $ (10\gamma)^r k$ & $ C \cdot 8^i  k_r /\epsilon_r$ \\ \hline
    \end{tabular}
\end{center}\caption{The main intuition is $k_r$ should shrink slightly faster than $\epsilon_r$ in each iteration. ``Our \cite{hikp12a}'' shows how to plugging our new idea into the original analysis of \cite{hikp12a}.}
\end{table}
\end{comment}


==> pairwise.tex <==
\section{Main Set Query}\label{sec:pairwise}

In this section, we present our set query data structure. We first give the construction of sketching matrix in Section~\ref{sec:pairwise_sketching_matrix_construction}. Then we show our new set query data structure in Section~\ref{sec:pairwise_algorithm}. We give an analysis of the data structure in Section~\ref{sec:pairwise_main_result}, whose correctness relies on a technical lemma on iterative loop, which is proved in Section~\ref{sec:pairwise_iterative_loop}.

\subsection{Construction of sketching matrix}\label{sec:pairwise_sketching_matrix_construction}

The sketching matrix used in our set query data structure consists of $\log k$ parts, where the $i$-th part ($i \in [\log k]$) of the sketching matrix corresponds to a count sketch data structure that hashes $n$ elements into $B_i$ bins. We defer the choice of $B_i$ to Section~\ref{sec:pairwise_algorithm}. We present the sketching matrix $\Phi$ below.

\begin{definition}[Sketching matrix $\Phi$]\label{def:pairwise_Phi}
For each $i\in [\log k]$, we choose $h_i : [n] \rightarrow [B_i]$ to be a pairwise independent hash function, and choose $\sigma_i : [n] \rightarrow \{-1,+1\}$ to be a pairwise independent hash function.

For each $i \in [\log k]$, we define \textsc{Count-Sketch} matrix $\Phi^{(i)} \in \R^{B_i \times n}$ as follows
\begin{align*}
\Phi^{(i)}_{j,l} =
\begin{cases}
 \sigma_i (l) & \mathrm{~if~} h_i(l) = j \\
 0 & \mathrm{~otherwise.~}
\end{cases}
\end{align*}
Let $m = \sum_{i=1}^{\log k} B_i$. We define matrix $\Phi \in \R^{ m \times n}$ as follows
\begin{align*}
\Phi =
\begin{bmatrix}
\Phi^{(1)} \\
\Phi^{(2)} \\
\cdots \\
\Phi^{(\log k)}
\end{bmatrix}.
\end{align*}
\end{definition}

\subsection{Algorithm}\label{sec:pairwise_algorithm}

Let $C$ be a sufficiently large constant, and $\gamma$ be a sufficiently small constant. For $i \in [\log k]$, let $k_i = k \gamma^i$ and $\epsilon_i = \epsilon (10\gamma)^i$. Let $B_i=C k_i / \epsilon_i$. The set query algorithm maintains the measurement $y=\Phi x$.

On update operation, the algorithm follows directly through the definition of sketching matrix $\Phi$. Namely, on \textsc{Update}$(i,\Delta)$, the algorithm finds the non-zero elements of the $i$-th column of $\Phi$, and update the measurement $y$ accordingly.

On query operation \textsc{Query}$(x,S)$, the recovery procedure uses $x'$ to record the current best approximation of $x$, and initially set $x' \leftarrow 0$. The procedure consists of $\log k$ iterations. In the $i$-th iteration, let $S_i \subseteq S$ denote the set of coordinates in $x$ that are yet to be recovered. Initially $S_1=S$.
Remind that sketching matrix $\Phi$ in Definition~\ref{def:pairwise_Phi} consists of $\log k$ parts, and the $i$-th part corresponds to a count sketch data structure with pair-wise independent hash function $h_i$ and random sign function $\sigma_i$.
In the $i$-th iteration of the set query algorithm,
\begin{align*}
T_i \leftarrow \left\{ j \in S_i ~\big|~ h_i^{-1}(j) \cap S_i = \emptyset \right\}.
\end{align*}
Intuitively the hash function $h_i$ maps $n$ elements into $B_i$ bins, for any $j \in S_i$, we have $j \in T_i$ if and only if $j$ does not collide with any other elements in $S_i$ (in that case, we say $j$ is isolated).

The procedure also maintains $y^{(i)}$, which is the measurement of the residual vector $x-x'$ (before the start of $i$-th iteration). After obtaining $T_i$, the procedure uses $y^{(i)}$ to estimate $x_j$ for every $j \in T_i$. Then the procedure updates $S_i$ and $x'$ accordingly. Finally, the algorithm outputs $x'$. Our iterative set query algorithm is presented in Algorithm~\ref{alg:pairwise_set_query}.

\begin{algorithm}[!h]
\begin{algorithmic}[1]\caption{Iterative set query}\label{alg:pairwise_set_query}
\Procedure{\textsc{IterativeSetQuery}}{$\epsilon,k$} \Comment{Theorem~\ref{thm:pairwise_set_query}}
	\State $C \leftarrow 20, \gamma \leftarrow 1/600$
	\For{$i=1 \to \log k$}
		\State $k_i \leftarrow k \gamma^i$, $\epsilon_i \leftarrow \epsilon (10\gamma)^i$
		\State $B_i \leftarrow C k_i / \epsilon_i $
	\EndFor
  \State $m \leftarrow \sum_{i=1}^{\log k} B_i$ \Comment{$m$ is the number of measurement}
	\State Construct matrix $\Phi$ according to Definition~\ref{def:pairwise_Phi} \Comment{$\Phi \in \R^{m \times n}$}
  \State $y \leftarrow 0$ \Comment{$y \in \R^m$}
	\Procedure{\textsc{Update}}{$i,\Delta$}
		\State $y \leftarrow y + \Delta \cdot (\Phi \cdot e_i)$
	\EndProcedure
	\Procedure{\textsc{Query}}{$x,S$}
		\State $S_1 \leftarrow S$
		\State $y^{(1)} \leftarrow y$
    \State $x' \leftarrow 0$ \Comment{$x' \in \R^n$ records an estimation of $x$}
		\For{$i=1 \to \log k$}
			\State Find $T_i \subseteq S_i$ such that for each $j\in T_i$, it is isolated from other coordinates in $S_i$
			\State $l \leftarrow \sum_{i'=1}^{i-1} B_{i'}$
			\State For each $j \in T_i$, compute $\wh{x}_j \leftarrow y^{(i)}_{l + h_i(j)} $
			\State $S_{i+1} \leftarrow S_i \backslash T_i$
			\State $y^{(i+1)} \leftarrow y^{(i)} -\Phi \wh{x}_{T_i} $
			\State $x' \leftarrow x' + \wh{x}_{T_i}$
		\EndFor
		\State \Return $x'$%$\{Z_j\}_{j \in T}$
    %\State Now $|S_i|\leq \frac{k}{\poly\log(k)}$, we can get $x_{S_i}$ through a simple count-sketch approach
	\EndProcedure
\EndProcedure
\end{algorithmic}
\end{algorithm}



\subsection{Analysis of iterative loop}\label{sec:pairwise_iterative_loop}

In this subsection, we characterize and prove two properties of the iterative loop in Algorithm~\ref{alg:pairwise_set_query}.
The first property states that with good probability, as $i$ increases, the size of $S_i$ shrinks by a factor of at least $1-\gamma$, and otherwise its size does not increase. This property is guaranteed by identification property of count sketch and our choice of parameters.
The second property states that with good probability, the estimation error in each round is small. This is guaranteed by estimation property of count sketch and our choice of parameters.
We formalize both properties in Lemma~\ref{lem:pairwise_induction} as follows. 

\begin{lemma}\label{lem:pairwise_induction}
Given parameters $\epsilon \in (0,1), k\geq 1 $, for each $i\in [\log k]$, we define
\begin{align*}
k_i = k \gamma^{i}, \epsilon_i = \epsilon (10 \gamma)^{i}, B_i = C \cdot k_i / \epsilon_i.
\end{align*}
For each $i\in [\log k]$, if
\begin{align*}
\forall j \in [i-1],  |S_{j+1 }| \leq \gamma |S_j|,
\end{align*}
and
\begin{align*}
\forall j \in [i-1], \sum_{t\in T_j} |x_t - \wh{x}_t|^2 \leq \epsilon \cdot 2^{-j} \| x_{\ov{S}} \|_2^2.
\end{align*}
Then we have : \\
{\rm Property (\RN{1}) :} With probability at least $1- \frac{1}{C\gamma} (10\gamma)^i$,
\begin{align*}
|S_{i+1}| \leq \gamma |S_i|,
\end{align*}
and otherwise $|S_{i+1}| \leq |S_i|$.\\
{\rm Property (\RN{2}) :} With probability at least $1- \frac{2}{C}(20\gamma)^i$,
\begin{align*}
\sum_{t\in T_i} | x_t - \wh{x}_t |^2 \leq \epsilon \cdot 2^{-i} \| x_{\ov{S}} \|_2^2.
\end{align*}
\end{lemma}
\begin{proof}

{\bf Proof of Property (\RN{1}).}

For each $i\in [\log k]$, for each $j \in S_i$, we use $Z_{i,j}$ to denote the boolean random variable where $Z_{i,j}=1$ if there exists a $j' \in S_i\backslash \{j\}$ such that $h_{i}(j) = h_{i}(j')$ and $Z_{i,j}=0$ otherwise. By the randomness of hash function $h_i$,
\begin{align*}
\Pr_{h_i} [ Z_{i,j} = 1 ] = \Pr_{h_i} [ j\text{~is~not~isolated~from~}S_i] \leq |S_i|/ B_i.
\end{align*}

By the statement of the lemma, we know that $|S_i| \leq \gamma^{i} k$ and $B_i = C k \gamma^{i} /\epsilon_i $, thus
\begin{align*}
\Pr_{h_i} [ Z_{i,j} = 1] \leq \gamma^{i} k / B_i \leq \epsilon_i / C.
\end{align*}

We define $Z_{i} = \sum_{j \in S_i} Z_{i,j}$. Next, we can show
\begin{align*}
 \E_{h_i} [Z_{i}] = \E_{h_i} [ | \{ j \in S_i ~|~ j \text{~is~not~isolated~from~} S_i \} | ]
 = \E_{h_i} \left[ \sum_{j \in S_i} Z_{i,j} \right]= ~ \sum_{j \in S_i } \E_{h_i} [ Z_{i,j} ] \leq |S_i| \epsilon_i /C,
\end{align*}

where the third step follows by linearity of expectation. Therefore,
\begin{align*}
\Pr_{h_i} [ Z_i \geq \gamma |S_i| ] \leq \E_{h_i} [Z_i] / (\gamma |S_i|) \leq |S_i| \epsilon_i / (C \gamma |S_i|) = \epsilon_i / (C \gamma),
\end{align*}

where the first step follows by Markov's inequality, and second step follows by $\E_{h_i} [Z_{i}]\leq |S_i| \epsilon_i /C$. This implies
\begin{align*}
\Pr[ |S_{i+1}| \geq \gamma |S_i| ] \leq  \epsilon  (10\gamma)^i / (C\gamma) \leq \frac{1}{C\gamma} (10\gamma)^i.
\end{align*}

{\bf Proof of Property (\RN{2}).}

We first define random variable $V_i$ to be
\begin{align*}
V_i = \sum_{l \in \left( \cup_{j \in S_i} h_i^{-1} (j) \right) \backslash S_i } |x_l^{(i)}|^2.
\end{align*}

That is, $x^{(i)}$ is the residual signal in the $i$-th round, and $V_i$ refers to the noise coordinates that are hashed to the same bins as coordinates in $S_i$. 

We can compute the expectation of $V_i$,
\begin{align*}
\E_{h_i} [ V_i ] = & ~ \E_{h_i} \left[ \sum_{l \in \left( \cup_{j \in S_i} h_i^{-1} (j) \right) \backslash S_i }  |x_l^{(i)}|^2 \right] \\
\leq & ~ k_i \| x_{\ov{S}_i}^{(i)} \|_2^2 / B_i \\
= & ~ \frac{  \epsilon_i }{C} \| x^{(i)}_{\ov{S}_i} \|_2^2 \\
= & ~ \frac{ (10 \gamma)^i \epsilon }{C} \| x^{(i)}_{\ov{S}_i} \|_2^2,
\end{align*}

where the first step follows by the fact that for each $l \in \ov{S_i}$, the probability that $l \in \left( \cup_{j \in S_i} h_i^{-1} (j) \right) \backslash S_i$ under the randomness of $h_i$ is $|S_i|/B_i \leq k_i/B_i$, the second and third step follow by definitions of $B_i$ and $\epsilon_i$, respectively.

By Markov's inequality, we have
\begin{align}\label{eq:sum_of_squares_is_upper_bounded}
\Pr_{h_i} \left[ V_i \geq \frac{1}{2} \cdot 10^{-i} \epsilon  \left\| x^{(i)}_{\ov{S}_i} \right\|_2^2 \right] \leq 2 \frac{ (100 \gamma)^i  }{C}.
\end{align}

In the following, we argue conditioned on the event that all elements in $T_i$ are isolated under $h_i$ and $V_i \leq 10^{-i} \epsilon \| x_{\ov{S}_i}^{(i)} \|_2^2 / 2$.

Recall the definition of $x^{(i)} \in \R^n$,
\begin{align}\label{eq:def_x^(i)}
x^{(i)} = x - \sum_{t \in S \backslash S_i} \wh{x}_t = x - \sum_{j=1}^{i} \sum_{t \in T_j} \wh{x}_t.
\end{align}


For any fixed $t \in T_i$, let $b = h_i(t)$. We have
\begin{align}\label{eq:bound_E_xt_whxt}
\E_{\sigma_i} \left [ | x_t - \wh{x}_t |^2 \right] = & ~ \E_{\sigma_i} \left[ \left| x_t - \sigma_{i}(t) \cdot  \sum_{l : h_i(l) = b} \sigma_{i}(l) x^{(i)}_l \right|^2 \right] \notag \\
= & ~ \E_{\sigma_i} \left[ \left| \sum_{l \in h_i^{-1}(b) \backslash \{t\} } \sigma_{i}(l) x^{(i)}_l \right|^2 \right] \notag \\
= & ~ \sum_{l \in h_i^{-1}(b) \backslash \{t\} } | x_l^{(i)} |_2^2,
\end{align}

where the first step follows by definition of $\hat{x}_t$ in Algorithm~\ref{alg:pairwise_set_query} and construction of sketching matrix $\Phi$ in Definition~\ref{def:pairwise_Phi},
the third step follows by pairwise independence property of random sign function $\sigma_i$.

We can upper bound $\E_{\sigma_i}[ \sum_{t \in T_i} |x_t - \wh{x}_t|^2 ]$ in the following way,
\begin{align}\label{eq:expectation_noise}
\E_{\sigma_i} \left[ \sum_{t \in T_i} |x_t - \wh{x}_t|^2 \right] = & ~ \sum_{t \in T_i} \sum_{l \in h_i^{-1}(t) \backslash \{t\} } | x_l^{(i)} |_2^2 & \text{~by~Eq.~\eqref{eq:bound_E_xt_whxt}} \notag \\
\leq & ~ \sum_{l \in \cup_{t\in S_i} h_i^{-1}(t) \backslash \{t\} } | x_l^{(i)} |_2^2 & \text{~by~definition~of~}T_i \notag \\
\leq & ~ \epsilon 10^{-i} \| x_{\ov{S}_i}^{(i)} \|_2^2 / 2 & \text{~by~Eq.~\eqref{eq:sum_of_squares_is_upper_bounded}} \notag \\
\leq & ~ \epsilon 10^{-i} \| x_{\ov{S}} \|_2^2 & \text{~by~Eq.~\eqref{eq:bound_norm_of_ov_S_i}}
\end{align}


\begin{comment}
and calculate the expected value of $V_i$ with respect to the randomness of the pairwise independent hash functions:

\begin{align}
\E V_i = \E \sum_{t \in S_i} \sum_{l \in h^{-1}(t) \setminus S_i} (x_l^{(i)})^2\\
 = \sum_{t \in S_i} \E\sum_{l \in h^{-1}(t) \setminus S_i} (x_l^{(i)})^2\\
\leq k_i \frac{1}{B_i} \|x_{\ov{S}_i}^{(i)}\|_2^2 = \epsilon_i/C \|x_{\ov{S}_i^{(i)}}\|_2^2,
\end{align}

since $|S_i| \leq k_i$, and

\[\E\sum_{l \in h^{-1}(t) \setminus S_i} (x_l^{(i)})^2 = \frac{1}{B_i} \|x_{\ov{S_i}^{(i)}}\|_2^2.\]


We apply Markov's inequality to $V_i$ to obtain

\begin{align}
\Pr \left[ V_i \geq 4^{-i} \epsilon/ C \|x_{\ov{S}_i}^{(i)}\|_2^2 \right] \\
\leq \frac{\epsilon_i/C \|x_{\ov{S}_i}^{(i)}|_2^2}{ 4^{-i} \epsilon/ C \|x_{\ov{S}_i}^{(i)}\|_2^2} \\
= (40\gamma)^i = 15^{-i}
\end{align}

We condition on the event that $\mathcal{W}_i: \{V_i < 4^{-i} \epsilon/ C \|x_{\ov{S}_i}^{(i)}\|_2^2 \}$, which happens with probability $1 - 15^{-i}$, and show how to upper bound $\E_{\sigma}[ \sum_{t \in T_i} |x_t - \wh{x}_t|^2 | \mathcal{W}_i]$:

 \begin{align}\label{eq:expectation_noise}
\E_{\sigma} \left[ \sum_{t \in T_i} |x_t - \wh{x}_t|^2| \mathcal{W}_i \right] \\
= \E_{\sigma} \left[ \sum_{t \in T_i} |x_t^{(i)} - \wh{x}_t^{(i)}|^2 | \mathcal{W}_i \right]\\
= \E_{\sigma} \left[ \sum_{t \in T_i} (\sum_{l \in h^{-1}_i(t) \setminus \{t\}} \sigma_{i,l} x_l^{(i)})^2 | \mathcal{W}_i \right]\\
= \E_{\sigma} \left[ \sum_{t \in T_i} (\sum_{l \in h^{-1}_i(t) \setminus S_i} \sigma_{i,l} x_l^{(i)})^2 | \mathcal{W}_i \right]\\
\leq  \E_{\sigma} \left[ \sum_{t \in S_i} (\sum_{l \in h^{-1}_i(t) \setminus S_i} \sigma_{i,l} x_l^{(i)})^2 | \mathcal{W}_i \right]\\
=  \sum_{t \in S_i}   \sum_{(l,l') \in (h^{-1}_i(t) \setminus S_i,h^{-1}_i(t) \setminus S_i)} \E_{\sigma} \left[ \sigma_{i,l} \sigma_{i,l'} x_{l}^{(i)} x_{l'}^{(i)} | \mathcal{W}_i  \right]\\
= \sum_{t \in S_i} \sum_{l \in h^{-1}_i(t) \setminus S_i} (x_l^{(i)})^2 \\
= V_i \leq 4^{-i} \epsilon/ C_i \|x_{\ov{S}_i}^{(i)} \|_2^2.
\end{align}
%We first show how to upper bound $|T_i| / B_i $,
%\begin{align}\label{eq:bound_T_i_over_B_i}
%\frac{|T_i|}{ B_i }
%\leq & ~ \frac{|S_i|}{ B_i} & \text{~by~} |T_i| \leq |S_i| \notag \\
%\leq & ~ \frac{\gamma^{i} k }{B_i}  & \text{~by~statement~of~Lemma} \notag \\
%= & ~  \frac{\gamma^{i} k }{ C \frac{k_i}{\epsilon_i} } & \text{~by~} B_i = C \frac{k_i}{\epsilon_i} \notag \\
%= & ~ \frac{\epsilon_i}{C} & \text{~by~} k_i = k \cdot \gamma^{i} \notag \\
%= & ~ \frac{1}{C} \epsilon (10 \gamma)^i & \text{~by~} \epsilon_i = \epsilon (10 \gamma)^i
%\end{align}

\end{comment}

%Let $b = h_i(t)$. Then
%\begin{align*}
%\E_{\sigma_i} \left [ | x_t - \wh{x}_t |^2 \right] = & ~ \E_{\sigma_i} \left[ \left| x_t - \sum_{l : h_i(l) = b} \sigma_{i,l} x^{(i)}_l \right|^2 \right] \\
%= & ~ \sum_{l \in h_i^{-1}(b) \backslash \{t\} } \| x_l^{(i)} \|_2^2 \\
%\end{align*}

%We can upper bound $\E_{\sigma_i}[ \sum_{t \in T_i} |x_t - \wh{x}_t|^2 ]$ in the following way,
%\begin{align}\label{eq:expectation_noise}
%\E_{\sigma_i} \left[ \sum_{t \in T_i} |x_t - \wh{x}_t|^2 \right] = & ~ \sum_{t \in T_i} \sum_{l \in h_i^{-1}(b) \backslash \{t\} } \| x_l^{(i)} \|_2^2 \notag \\
%\leq & ~ \sum_{t \in S_i} \sum_{l \in h_i^{-1}(b) \backslash \{t\} } \| x_l^{(i)} \|_2^2 \notag \\
%\leq & ~ \epsilon 2^{-i} \| x_{\ov{S}_i}^{(i)} \|_2^2 / 2 \notag \\
%\leq & ~ \epsilon 2^{-i} \| x_{\ov{S}} \|_2^2 & \text{~by~Eq.~\eqref{eq:bound_norm_of_ov_S_i}}
% \leq \frac{|T_i|}{ B_i } \cdot \| x_{\ov{S}_i}^{(i)} \|_2^2.
%\end{align}
%\begin{comment}
%We first show how to upper bound $|T_i| / B_i $,
%\begin{align}\label{eq:bound_T_i_over_B_i}
%\frac{|T_i|}{ B_i }
%\leq & ~ \frac{|S_i|}{ B_i} & \text{~by~} |T_i| \leq |S_i| \notag \\
%\leq & ~ \frac{\gamma^{i} k }{B_i}  & \text{~by~statement~of~Lemma} \notag \\
%= & ~  \frac{\gamma^{i} k }{ C \frac{k_i}{\epsilon_i} } & \text{~by~} B_i = C \frac{k_i}{\epsilon_i} \notag \\
%= & ~ \frac{\epsilon_i}{C} & \text{~by~} k_i = k \cdot \gamma^{i} \notag \\
%= & ~ \frac{1}{C} \epsilon (10 \gamma)^i & \text{~by~} \epsilon_i = \epsilon (10 \gamma)^i
%\end{align}
%\end{comment}
Second, we show how to upper bound $\| x_{\ov{S}_i}^{(i)} \|_2^2$,
\begin{align}\label{eq:bound_norm_of_ov_S_i}
\| x_{\ov{S}_i}^{(i)} \|_2^2
 = & ~ \| x_{\ov{S} \cup S \backslash S_i}^{(i)} \|_2^2 & \text{~by~} \ov{S_i} = \ov{S} \cup S \backslash S_i \notag \\
 = & ~ \| x_{\ov{S}}^{(i)} \|_2^2 + \| x_{S \backslash S_i}^{(i)} \|_2^2 & \text{~by~} \ov{S} \cap (S \backslash S_i) = \emptyset \notag \\
 = & ~ \| x_{\ov{S}} \|_2^2 + \| x_{S \backslash S_i}^{(i)} \|_2^2 & \text{~by~}  x_{\ov{S}}^{(i)} = x_{\ov{S}} \notag  \\
  = & ~ \| x_{\ov{S}} \|_2^2 + \sum_{j=1}^{i-1} \| x_{T_j}^{(i)} \|_2^2 & \text{~by~} S\backslash S_i = T_1 \cup T_2 \cup \cdots \cup T_{i-1} \notag \\
  = & ~ \| x_{\ov{S}} \|_2^2 + \sum_{j=1}^{i-1} \sum_{t\in T_j} | x_t -\wh{x}_t |^2 & \text{~by~Eq.~\eqref{eq:def_x^(i)}} \notag \\
  \leq & ~ \| x_{\ov{S}} \|_2^2 + \sum_{j=1}^{i-1} \epsilon 2^{-j} \| x_{\ov{S}} \|_2^2 & \text{~by~statement~of~Lemma} \notag \\
  \leq & ~ 2 \| x_{\ov{S}} \|_2^2. & \text{by~geometric~sum}
\end{align}



Using Markov's inequality $\Pr[X \geq a ]\leq \E[X] /a$, we have
\begin{align*}
\Pr \left[  \sum_{t \in T_i} |x_t - \wh{x}_t|^2 \geq \epsilon 2^{-i} \| x_{\ov{S}} \|_2^2 \right] \leq 5^{-i}.
\end{align*}

Therefore, we complete the proof.
\end{proof}



\subsection{Main result}\label{sec:pairwise_main_result}

In this section, we prove the correctness of our iterative set query algorithm, as well as justify the claimed space complexity, update time and query time. At the core of correctness is an analysis of the iterative loop, which is given as Lemma~\ref{lem:pairwise_induction} in Section~\ref{sec:pairwise_iterative_loop}.

\begin{theorem}\label{thm:pairwise_set_query}
Let $m=O(k/\epsilon)$. We can give a randomized construction of a matrix $\Phi \in \R^{m\times n}$ (Definition~\ref{def:pairwise_Phi}) such that for each set $S \subseteq [n]$, $|S| \leq k$, and for each vector $x \in \R^n$, there is an algorithm (Algorithm~\ref{alg:pairwise_set_query}) that takes $\Phi x$ as its input, and finds $x'\in \R^k$ such that
\begin{align*}
\| x' - x_S \|_2^2 \leq \epsilon \| x_{[n] \backslash S} \|_2^2
\end{align*}
holds with probability $9/10$. The space to store matrix $\Phi$ is $O(\log k)$ words. The columns of matrix $\Phi$ are $2$-wise independent. The update time is $O(\log k)$. The decoding time is $O(k \log k)$.
\end{theorem}
\begin{proof}

Our proof is based on properties of the iterative loop in Algorithm~\ref{alg:pairwise_set_query}. The properties are formulated as Lemma~\ref{lem:pairwise_induction} in Section~\ref{sec:pairwise_iterative_loop}. In summary, property (I) in Lemma~\ref{lem:pairwise_induction} shows that with good probability, as $i$ increases, the size of $S_i$ (i.e. the set of coordinates in $S$ that yet to be recovered at the beginning of $i$-th round) shrinks by a constant factor, and otherwise its size does not increase. Property (II) in Lemma~\ref{lem:pairwise_induction} shows that with good probability, the estimation error in each round is small. 

{\bf Proof of success probability.}
It follows by recursively applying Lemma~\ref{lem:pairwise_induction}. By union bound, the failure probability is bounded by
\begin{align*}
\sum_{i=1}^{\log k} \left( \frac{1}{C\gamma} (10\gamma)^i + \frac{2}{C} (20\gamma)^i \right) < 1/10,
\end{align*}

which follows from geometric sum and the choice of parameters.

{\bf Proof of estimation error.}
\begin{align*}
\|x' - x_S\|_2^2 \leq
\sum_{i=1}^{\log k} \sum_{t\in T_i} | x_t - \wh{x}_t |^2 \leq
\sum_{i=1}^{\log k} \epsilon \cdot 2^{-i} \| x_{\ov{S}} \|_2^2 \leq
\epsilon \| x_{\ov{S}} \|_2^2.
\end{align*}

{\bf Proof of space to store $\Phi$.}
Since for each $i\in [\log k]$, $\Phi^{(i)}$ only uses $2$ pairwise independent hash functions, the space to store matrix $\Phi$ is $O(\log k)$ words.

{\bf Proof of update time.}
Upon update $(j, \Delta)$, for each $\Phi^{(i)}$, the algorithm only needs to update one measurement (located at $h_i(j)$).
Therefore, the update time is $O(\log k)$. Since every element of the matrix can be computed in $O(1)$ time.

{\bf Proof of query time.}
First of all, we note that the step in Line 18 can be performed in $O(|S_i|)$ time upon query, since we can check every $j \in S_i$, and mark the buckets that have more than one $j$ hashed to them; in the next step we just keep only those coordinates $j$ that are hashed to exactly one bucket. Recursively applying Lemma~\ref{lem:pairwise_induction}, we have with constant probability, such that for all $i\in [\log k]$, $|S_{i+1}| \leq \gamma |S_{i}|$. It implies that for all $i \in [\log k]$, $|S_i| \leq \gamma^{i-1} |S_1| \leq \gamma^{i-1} k$. Note that in iteration $i \in [\log k]$, we need $O(|S_i|)$ update time. Therefore, overall the iterations, the time of this part is
\begin{align*}
\sum_{i=1}^{\log k} O(|S_i|) \leq O \left( \sum_{i=1}^{\log k} \gamma^{i-1} k \right) = O(k),
\end{align*}
where the last step follows by the choice of $\gamma$.

We know that $\| z\|_0 = O(k)$ and $|T_i| = O(k)$. Thus, in each iteration, the time of doing step $y^{(i+1)} \leftarrow y^{(i)} - \Phi Z_{T_i}$ requires $O(k)$ time. Thus the subtraction time over all iterations is $O(k\log k)$, since there are $O(\log k)$ iterations. Putting it together, we get $O(k\log k)$ query time.

%On iteration $i$ we use the count-sketch to recover up to $|S_i|$ coordinates, and remove their magnitude from the count-sketch for iteration $i+1, i+2, \ldots$, and thus it takes up to $|S_i| \log\log k$ time.
%Across all the iterations, the query time is $O(\sum_{i=1}^{\log\log k} |S_i| \log\log k) = O(k \log\log k)$.

%To estimate the magnitudes of coordinates in $S_{\log\log k}$, we use a separate count-sketch. Each coordinate is estimated by taking a median of $O(\log k)$ values. So this step takes $O(|S_{\log\log k}| \cdot \log k)=O(k)$ time.
\end{proof}

